Covering Cracks in Content Moderation: Delexicalized Distant Supervision for Illicit Drug Jargon Detection

In light of rising drug-related concerns and the increasing role of social media, sales and discussions of illicit drugs have become commonplace online. Social media platforms hosting user-generated content must therefore perform content moderation, which is a difficult task due to the vast amount of jargon used in drug discussions. Previous works on drug jargon detection were limited to extracting a list of terms, but these approaches have fundamental problems in practical application. First, they are trivially evaded using word substitutions. Second, they cannot distinguish whether euphemistic terms such as "pot" or "crack" are being used as drugs or in their benign meanings. We argue that drug content moderation should be done using contexts rather than relying on a banlist. However, manually annotated datasets for training such a task are not only expensive but also prone to becoming obsolete. We present JEDIS, a framework for detecting illicit drug jargon terms by analyzing their contexts. JEDIS utilizes a novel approach that combines distant supervision and delexicalization, which allows JEDIS to be trained without human-labeled data while being robust to new terms and euphemisms. Experiments on two manually annotated datasets show JEDIS significantly outperforms state-of-the-art word-based baselines in terms of F1-score and detection coverage in drug jargon detection. We also conduct qualitative analysis that demonstrates JEDIS is robust against pitfalls faced by existing approaches.

==> Sections/2.5_Problem.tex <==
% \section{Problem Definition}
% % \begin{figure*}[t]
% %     \centering
% %     \includegraphics[width=0.99\linewidth]{Figures/Approach_overview.pdf}
% %     \caption{Detection Approach Overview}
% %     \label{fig:apporach_overview}
% % \end{figure*}
% To avoid confusion, we clearly define the terms used in this paper. Note that these terms are often used inconsistently or interchangeably between works.
% We define \textbf{drug jargon} as words used to refer to illicit drug substances and abused legal drug substances. This can include both explicit substance names (e.g., \textit{MDMA}, \textit{ketamine}) and street names (e.g., \textit{Molly}, \textit{ket}). Some jargon terms are \textbf{euphemisms} (e.g., \textit{speed}, \textit{pot}), polysemous words that have alternate innocuous meanings. It should be noted that slang terms are not necessarily euphemisms (\textit{fent}, for instance is just a shortened version of \textit{fentanyl}). Similarly, drug euphemisms are not always used as drug jargon, even in an illegal drug context (e.g., ``[product from dealer] had good \textit{speed} of delivery"). We formalize the task of \textbf{drug jargon detection} as a binary classification problem. Given a context and a word in the context, a system must determine whether the word is used as a drug jargon in the context. This task is contrary to \textbf{drug jargon extraction}
% %, which was performed by existing word-based systems for content moderation. In extraction task, a system extracts drug jargon in the form of a list after investigating the entire corpus.
% of past works, which is focused on extracting a list of drug jargon from a target corpus.

==> Sections/6_Jargon_Extraction_Evaluation.tex <==
\section{Drug Jargon Extraction Evaluation}
\label{extraction}
We have shown experiments that suggest effective automatic content moderation must be done using contexts.
However, jargon extraction can still be of value in moderating content.
For instance, a dictionary of previously unknown drug terms can offer assistance to human moderators that lack domain knowledge.
Therefore, we test the possibility of using our delexicalized system in the task of extracting drug jargon terms from a corpus.
In this task, we use the four word-based systems trained in Section~\ref{detection_evaluation} as the baselines.
%For each moderation system, we use trained model in Section~\ref{}.

% \input{Tables/evaluation_table_word_precision}
% \vspace{0.1cm}
% \noindent\textbf{Top100 jargon list construction.}
\subsection{Drug Jargon List Construction}
To extract a list of drug jargon from a corpus, we can apply our drug jargon detection system to all sentences in the entire corpus.
To score a word candidate, we count both prediction frequency $F_{pred}$ (how many times the word was positively predicted as drug jargon) and prediction ratio $R_{pred}$ (the number of positive predictions divided by the number of total predictions made) of the word. Our score is given by the following formula.
\begin{align}
    \textit{Score} = F_{pred}*{R_{pred}}^{n}
\end{align}
We have a weighing parameter $n$ to balance the factors, which can be controlled to be more or less sensitive to frequently occurring words. For our evaluation, we used $n = 2$ and extracted the top 100 words.

For all the baselines, we also apply them to the entire corpus for extracting drug jargon lists.
In the case of Word2Vec, we select the top 100 drug jargon sorted by the cosine similarity of word embedding with seed terms. For CantReader and Zhu et al., we extract the top 100 jargon sorted by the extraction probability outlined in the respective papers~\cite{cantreader,zhu2021self}.
We present the top 100 extracted jargon list of each system on Table~\ref{tab:top100_word_list} in the Appendix~\ref{appendix}.


\input{Tables/qualitative_analysis}
% \input{Tables/word_based_comparison}
\subsection{Quantitative Evaluation}
%For evaluation, we utilize the entire corpus as a reference to evaluate words.
In the evaluation step, we manually investigate if the word is used as drug jargon in the corpus, using the guidelines in Appendix~\ref{appendix}. 
%Although our approach is focused on word contexts, we test if our system can be applied to extracting jargon terms from a corpus.
Table~\ref{tab:evaluation2} shows the results for our jargon extraction evaluation in the perspective of precision. Overall, the Word2Vec model shows the best performance for both corpora. Surprisingly, \model{} shows comparable performance, showing the second best performance in most settings and the best performance in a few. Moreover, it outperformed both the euphemism-aware jargon extraction systems. It is possible that attempting to find euphemisms can lead to a more imprecise collection. The results suggest that our delexicalized jargon detection system, \model{} can also be used effectively as a jargon extraction system, even when the system is trained in a lexicon-agnostic manner. A noteworthy observation is that both Word2Vec and our system produce consistently high precision at values up to $K=100$, while the euphemism-aware systems suffer a large performance drop as K increases. This suggests these methods can find more correct terms beyond the evaluated 100 terms.
% \input{Tables/qualitative_analysis}
% \input{Tables/word_based_comparison}
\subsection{Qualitative Evaluation}
\label{qaulitative_evaluation}



For each moderation system, we further examine the produced word list to find limitations. 
% We compare \model{} with existing word-based systems in Table~\ref{tab:word_based_comparision}.
We further identify cases of failure of the systems and present examples as shown in Table~\ref{tab:qaulitative_examples}.

The Word2Vec systems showed high overall performance in the precision metrics.
However, it was suspected that it may not be able to effectively identify euphemisms.
After comparing with the list produced by other methods, we find that the Word2Vec list misses many euphemisms found by other approaches.
For instance, Word2Vec could not identify \textit{weed}, \textit{speed}, \textit{lucy}, \textit{spice}, and \textit{crack}, which were all identified by both \model{} and Zhu et al.'s system.
Word2Vec assumes a single meaning for each word, which can make it less effective in dealing with polysemous euphemisms.
Therefore, adversaries can easily exploit Word2Vec's weakness by using common words as euphemisms.

CantReader showed low overall precision with many false positives.
CantReader is designed to find euphemisms by finding words that are used differently across corpora.
However, with the exception of \textit{weed}, it was also not able to find the above euphemisms that Word2Vec failed to find.
The CantReader word list reveals that many false positives came from misspelled non-Jargon words, such as \textit{comfused}, \textit{enver}, and \textit{niceeeeee}.
By design, the system gives infrequent words high scores since they may be characteristic to the target corpus.
However, this suggests it is unsuitable to use in user-generated texts that can often contain typos.

Zhu et al.'s system is based on making a finetuned BERT model that predicts how likely each word is able to fit a context.
However, this model is only capable of doing this with words within its limited wordpiece vocabulary.
Although the system is capable of finding many euphemistic terms, words that are not contained in BERT's vocabulary cannot be detected by this system, even if the corpus clearly uses it as drug jargon.
Terms like \textit{valium}, \textit{ambien}, \textit{diazepam}, \textit{oxy}, and \textit{focalin} were terms found by Word2Vec and \model{}, but were not found by Zhu et al.'s system because they are not in BERT's vocabulary.
Furthermore, this limitation causes false positives.
BERT splits out-of-vocabulary words into wordpieces, so unknown words (like \textit{meth}) will be represented as a combination of two words (\textit{met} and \textit{\#\#h}).
The false positives \textit{met}, \textit{add}, and \textit{mx} may indicate \textit{meth}, \textit{adderall}, and \textit{mxe}.
This highlights the limitation that the system cannot predict out-of-vocabulary words correctly, even when the model has sufficiently learned them.

Our system judges words by how their contexts appear to be, rather than the words themselves. Therefore, a common cause of false positives was words that can be used to replace illicit drugs in most contexts. The words \textit{product} and \textit{stuff} are not drug words, but can be used to reference a drug.
Another type of error was legal drugs that are often discussed in similar ways to illicit drugs, such as \textit{alcohol} and \textit{caffeine}.
%Similar errors could occur in other systems, but since our delexicalized system cannot recognize benign words, such errors were more common.
However, these errors were common in other systems as well, suggesting it is a general linguistic limitation.
We discuss this limitation further in Section~\ref{challenges}.
\model{}, unlike other baselines, had no significant systematic failures in recall.
% In fact, since \model{} is not bound words from the corpus, the same system can apply to unseen words from other sources.
%Terms found by other systems but not found in our top-100, such as \textit{heroine}, \textit{dex}, and \textit{percs}, were found later down in the list (\#188, \#104, \#141).
Although Word2Vec had slightly higher precision scores, qualitative analysis suggests \model{} has better recall and overall performance.




==> Tables/comparison_word_set.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[t]
\caption{Top 30 most frequent nouns in STMS and non-STMS. \textit{STMS only} and \textit{non-STMS only} contain words that only appear in each set's top 30 frequent words. \textit{Both} contains words that are included in both sets.}
\label{tab:comparision_wordset}
\normalsize
\begin{subtable}{\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular} {P{0.14\linewidth}P{0.13\linewidth}|P{0.14\linewidth}P{0.14\linewidth}P{0.17\linewidth}|P{0.14\linewidth}P{0.16\linewidth}}
            \toprule
            \multicolumn{2}{c}{\textbf{STMS only}}    & \multicolumn{3}{c}{\textbf{Both}}    & \multicolumn{2}{c}{\textbf{non-STMS only}}  \\ 
            \midrule
            effect & \hspace{-0.2cm}pill	& time & drug & day   & bitcoin & btc     \\
            mg & \hspace{-0.2cm}month   &	friend & vendor & experience   & price & wallet      \\
            night & \hspace{-0.2cm}tab & trip & people	& use	    & money & someone    \\
            gram & \hspace{-0.2cm}dose   & anyone & order & year   & bitcoins & \hspace{-0.2cm}transaction   \\
            weed & \hspace{-0.2cm}test 	& hour & week & thing    & anything & market      \\
            amount &    & lot & way & something	    & bit  &       \\
            &   & question &  & & &           \\\bottomrule
        \end{tabular}%
    }
\vspace{0.03cm}
\caption{Reddit Drug corpus}
\end{subtable}
\normalsize
\begin{subtable}{\linewidth}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular} {P{0.14\linewidth}P{0.13\linewidth}|P{0.14\linewidth}P{0.14\linewidth}P{0.17\linewidth}|P{0.14\linewidth}P{0.16\linewidth}}
            \toprule
            \multicolumn{2}{c}{\textbf{STMS only}}    & \multicolumn{3}{c}{\textbf{Both}}    & \multicolumn{2}{c}{\textbf{non-STMS only}}  \\ 
            \midrule
            quality & \hspace{-0.2cm}pill	& order & time & vendor   & post & package     \\
            gram & \hspace{-0.42cm}experience   &	people & drug & day   & account & money      \\
            trip & \hspace{-0.2cm}effect & price & way	& sr	    & anything & message    \\
            test & \hspace{-0.2cm}pure   & thing & use & product   & forum & btc   \\
            year &  	& lot & anyone & something    & pgp &       \\
            &     & review & week & look	    & &         \\
            &   & bit &hour  &someone & &           \\\bottomrule
        \end{tabular}%
    }
\vspace{0.03cm}
\caption{Silk Road Forum corpus}
\end{subtable}
\end{table}

        % \begin{tabular} {p{0.14\linewidth}p{0.14\linewidth}|p{0.14\linewidth}p{0.14\linewidth}p{0.14\linewidth}|p{0.14\linewidth}p{0.14\linewidth}}

% \begin{table}[t]
% \caption{Most frequent nouns in STMS and non-STMS}
% % \footnotesize
% \begin{subtable}{\linewidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular} {cc|ccc|cc}
%             \toprule
%             \multicolumn{2}{c}{\textbf{STMS}}    & \multicolumn{3}{c}{\textbf{Intersection}}    & \multicolumn{2}{c}{\textbf{non-STMS}}  \\ 
%             \midrule
%             effect & pill	& time & drug & day   & bitcoin & btc     \\
%             mg & month   &	friend & vendor & experience   & price & wallet      \\
%             night & tab & trip & people	& use	    & money & someone    \\
%             gram &dose   & anyone & order & year   & bitcoins & transaction   \\
%             weed & test 	& hour & week & thing    & anything & market      \\
%             amount &    & lot & way & something	    & bit  &       \\
%             &   & question &  & & &           \\\bottomrule
%         \end{tabular}%
%     }
% \vspace{0.03cm}
% \caption{Reddit Drug dataset}
% \end{subtable}
% \begin{subtable}{\linewidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular} {cc|ccc|cc}
%             \toprule
%             \multicolumn{2}{c}{\textbf{STMS}}    & \multicolumn{3}{c}{\textbf{Intersection}}    & \multicolumn{2}{c}{\textbf{non-STMS}}  \\ 
%             \midrule
%             quality & pill	& order & time & vendor   & post & package     \\
%             gram & experience   &	people & drug & day   & account & money      \\
%             trip & effect & price & way	& sr	    & anything & message    \\
%             test & pure   & thing & use & product   & forum & btc   \\
%             year &  	& lot & anyone & something    & pgp &       \\
%             &     & review & week & look	    & &         \\
%             &   & bit &hour  &someone & &           \\\bottomrule
%         \end{tabular}%
%     }
% \vspace{0.03cm}
% \caption{Silk Road1 Forum dataset}
% \end{subtable}
% \label{comparision_wordset}
% \end{table}

==> Tables/data_preparation_algorithm_1.tex <==
\begin{algorithm2e}[t]
\DontPrintSemicolon
\caption{Data Processing, Filtering, Splitting}
\label{alg:data_preparation1}
\KwIn{Drug Seed Terms $T$, Training Corpus $C$}
\KwOut{Seed Term Mentioned Sentences $STMS$,\\
\hspace{1.35cm}$non$-$STMS$}
\For {$s \in  sent\_tokenize(C)$}{
    $s \gets remove\_nonASCII(s)$ \;
    $s \gets remove\_HTML(s)$ \;
    $S_{Processed}.append(s)$ \;
    }
\For {$s \in S_{Processed}$}{
    \If{$length(BERT\_tokenize(s)) \le 128$}{
        \If{$length(s.split()) > 5$}{
            $S_{Filtered}.append(s)$\;
            }
        }
    }
\For {$s \in S_{Filtered}$}{
    $stms \gets 0$\;
    \For{$t \in T$}{
       \If {$(?\hspace{-0.1cm}<!\backslash w)t(?!\backslash w) \in s.lower()$}{
        $stms \gets 1$\;
        $break\;$
            }
        }
    \eIf{$stms = 1$}{$STMS.append(s)$\;}
    {$non$-$STMS.append(s)$\;}
    }
\Return $STMS$, $non$-$STMS$\;
\end{algorithm2e}



% \begin{algorithm}[H]
%     \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%     \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \caption{Data Preparation}
%     \begin{algorithmic}[1]
%         \REQUIRE Drug Seed Terms $T$, Training Corpus $C$; \\
%         \ENSURE  Training Dataset $D$ \\
%         \FOR {$s \in  sent\_tokenize(C)$}
%             \STATE $s \gets remove\_nonASCII(s)$
%             \STATE $s \gets remove\_HTML(s)$
%             \STATE $S_{Processed}.append(s)$
%         \ENDFOR
%         \FOR {$s \in S_{Processed}$}
%             \IF{$length(word\_tokenize(s)) \le 128$}
%                 \IF{$length(s.split()) > 5$}
%                     \STATE $S_{Filtered}.append(s)$
%                 \ENDIF
%             \ENDIF
%         \ENDFOR
%         \FOR {$s \in S_{Filtered}$}
%             \STATE $W \gets word\_tokenize(s)$
%             \FOR {$(ind, w) \in enumerate(W)$}
%                 \IF {$w.lower() \in T$}
%                     \STATE $W^{\prime} \gets W.copy()$
%                     \STATE $W^{\prime}[ind] \gets [MASK]$
%                     \STATE $D.append(('\;'.join(W^{\prime}),1))$
%                 \ELSIF {$Is\_Noun(w)$\textbf{ and }$Is\_AlNum(w)$}
%                     \STATE $W^{\prime} \gets W.copy()$
%                     \STATE $W^{\prime}[ind] \gets [MASK]$
%                     \STATE $D.append(('\;'.join(W^{\prime}),0))$
%                     % \ENDIF
%                 \ENDIF
%             \ENDFOR
%         \ENDFOR
%         \STATE \textbf{return} $D$
%     \end{algorithmic}
%     \label{alg:data_preparation}
% \end{algorithm}




==> Tables/data_preparation_algorithm_2.tex <==
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{black}{#1}}
\SetCommentSty{mycommfont}
 
% \begin{algorithm2e}[t]
% \DontPrintSemicolon
% \caption{Masking and Negative Sampling}
% \label{alg:data_preparation2}
% % \algorithmfootnote{$y_0$ denotes the initial value.}
% \KwIn{Drug Seed Terms $\mathcal{T}$, $STMS$, $non$-$STMS$,\\
% Negative Sampling Ratio of STMS $\mathcal{R}_{STMS}$,\\
% Negative Sampling Ratio of non-STMS $\mathcal{R}_{nonSTMS}$}
% \KwOut{Training Dataset $\mathcal{D}$}
% $cnt_{pos} \gets 0$\;
% \For {$s \in STMS$}{
%     $W \gets word\_tokenize(s)$\;
%     $Neg_{tmp} \gets [\:\:] $\;
%     \For {$(ind, w) \in enumerate(W)$}{
%         \If {$w.lower() \in \mathcal{T}$}{
%             $W^{\prime} \gets W.copy()$\;
%              $W^{\prime}[ind] \gets [MASK]$\;
%              $\mathcal{D}.append(('\:\:'.join(W^{\prime}),\textbf{1}))$\;
%              $cnt_{pos} \mathrel{+}= 1$
%              }
             
%         \ElseIf {$isNoun(w)$\textbf{ and }$isAlNum(w)$}{
%             $W^{\prime} \gets W.copy()$\;
%             $W^{\prime}[ind] \gets [MASK]$\;
%             $Neg_{tmp}.append(('\:\:'.join(W^{\prime}),\textbf{0}))$\;
%             }
%         }
%     $\mathcal{D}.extend(Sample(Neg_{tmp}, \mathcal{R}_{STMS}))$\; 
%     % \tcc*{$Sample(L,n)$ denotes a procedure of sampling n data from list L.}
%     % \tcc{iterate over all training examples}
% }
% $S_{non} \gets Sample(non$-$STMS,\mathcal{R}_{nonSTMS}*cnt_{pos})$\;
% \For {$s \in S_{non}$}{
%     $W \gets word\_tokenize(s)$\;
%     $Neg_{tmp} \gets [\:\:] $\;
%     \For {$(ind, w) \in enumerate(W)$}{
%         \If {$isNoun(w)$\textbf{ and }$isAlNum(w)$}{
%             $W^{\prime} \gets W.copy()$\;
%             $W^{\prime}[ind] \gets [MASK]$\;
%             $Neg_{tmp}.append(('\:\:'.join(W^{\prime}),\textbf{0}))$\;
%             }
%         }
%     $\mathcal{D}.append(Sample(Neg_{tmp}, 1))$\;
% }
% \Return $\mathcal{D}$\;
% \end{algorithm2e}


\begin{algorithm2e}
\noindent\begin{minipage}{\linewidth}
\renewcommand\footnoterule{}
\DontPrintSemicolon
\caption{Masking and Negative Sampling}
\setcounter{AlgoLine}{0}
\label{alg:data_preparation2}
% \algorithmfootnote{$y_0$ denotes the initial value.}
\KwIn{Drug Seed Terms $\mathcal{T}$, $STMS$, $non$-$STMS$,\\
Negative Sampling Ratio of STMS $\mathcal{R}_{STMS}$,\\
Negative Sampling Ratio of non-STMS $\mathcal{R}_{nonSTMS}$}
\KwOut{Training Dataset $\mathcal{D}$}
$cnt_{pos} \gets 0$\;
\For {$s \in STMS$}{
    $W \gets word\_tokenize(s)$\;
    $Neg_{tmp} \gets [\:\:] $\;
    \For {$(ind, w) \in enumerate(W)$}{
        \If {$w.lower() \in \mathcal{T}$}{
            $W^{\prime} \gets W.copy()$\;
             $W^{\prime}[ind] \gets [MASK]$\;
             $\mathcal{D}.append(('\:\:'.join(W^{\prime}),\textbf{1}))$\;
             $cnt_{pos} \mathrel{+}= 1$
             }
             
        \ElseIf {$isNoun(w)$\textbf{ and }$isAlNum(w)$}{
            $W^{\prime} \gets W.copy()$\;
            $W^{\prime}[ind] \gets [MASK]$\;
            $Neg_{tmp}.append(('\:\:'.join(W^{\prime}),\textbf{0}))$\;
            }
        }
    $\mathcal{D}.extend(Sample(Neg_{tmp}, \mathcal{R}_{STMS})~\footnote{$Sample(L,n)$ denotes sampling n data from a list L.})$\; 
    % \tcc*{$Sample(L,n)$ denotes a procedure of sampling n data from list L.}
    % \tcc{iterate over all training examples}
}
$S_{non} \gets Sample(non$-$STMS,\mathcal{R}_{nonSTMS}*cnt_{pos})$\;
\For {$s \in S_{non}$}{
    $W \gets word\_tokenize(s)$\;
    $Neg_{tmp} \gets [\:\:] $\;
    \For {$(ind, w) \in enumerate(W)$}{
        \If {$isNoun(w)$\textbf{ and }$isAlNum(w)$}{
            $W^{\prime} \gets W.copy()$\;
            $W^{\prime}[ind] \gets [MASK]$\;
            $Neg_{tmp}.append(('\:\:'.join(W^{\prime}),\textbf{0}))$\;
            }
        }
    $\mathcal{D}.append(Sample(Neg_{tmp}, 1))$\;
}
\Return $\mathcal{D}$\;
\end{minipage}
\end{algorithm2e}



==> Tables/drug_seed_terms.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Drug seed terms extracted from DEA publication.}
%     % \footnotesize
%     \scriptsize
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular} {c c c c c c c c}
%             \toprule
%             \multicolumn{8}{c}{\textbf{Drug Seed Terms}} \\
%             \midrule
%             adderall & alprazolam & amphetamine & clonazepam & cocaine & concerta & daytrana & dilaudid \\
%             ecstasy & fentanyl & flunitrazepam & ghb & heroin & hydrocodone & hydromorphone & ketalar \\
%             ketamine & khat & klonopin & lorcet & lsd & marijuana & mdma & mescaline \\
%             methamphetamine & methylphenidate & molly & morphine & norco & opium & oxaydo & oxycodone \\
%             oxycontin & pcp & percocet & peyote & phencyclidine & promethazine & ritalin & rohypnol \\
%             roxicodone & steroids & suboxone & u-47700 & vicodin & xanax \\
%             \bottomrule   
%         \end{tabular}
%     }
%     \label{tab:drug_seed_terms}
% \end{table*}


\begin{table*}[t]
    \centering
    \caption{Drug seed terms extracted from the DEA report.}
    % \footnotesize
    % \scriptsize
    \resizebox{0.9\linewidth}{!}{%
        \begin{tabular} {c c c c c c c}
            \toprule
            \multicolumn{7}{c}{\textbf{Drug Seed Terms}} \\
            \midrule
            adderall & alprazolam & amphetamine & clonazepam & cocaine & concerta & daytrana \\
            dilaudid & ecstasy & fentanyl & flunitrazepam & ghb & heroin & hydrocodone \\
            hydromorphone & ketalar & ketamine & khat & klonopin & lorcet & lsd \\
            marijuana & mdma & mescaline& methamphetamine & methylphenidate & molly & morphine \\
            norco & opium & oxaydo & oxycodone & oxycontin & pcp & percocet \\
            peyote & phencyclidine & promethazine & ritalin & rohypnol & roxicodone & steroids \\
            suboxone & u-47700 & vicodin & xanax \\
            \bottomrule   
        \end{tabular}
    }
    \label{tab:drug_seed_terms}
\end{table*}




==> Tables/evaluation_table_word_precision.tex <==
\begin{table*}[t]
    \centering
    \caption{Precision of top K (P@K) extracted words. Boldface represents best performance and underline represents second-best performance.}
    \small
    % \resizebox{0.7\linewidth}{!}{%
        \begin{tabular} {l c c c c c c c c c}
            \toprule
            &   \multicolumn{4}{c}{\textbf{Reddit Drug}}  &  &   \multicolumn{4}{c}{\textbf{Silk Road Forum}}   \\ \cmidrule{2-5}\cmidrule{7-10}
            &   \textbf{P@10}  & \textbf{P@30}   & \textbf{P@50} & \textbf{P@100} &   & \textbf{P@10}  & \textbf{P@30}   & \textbf{P@50} & \textbf{P@100} \\
            \midrule
            \textbf{Word2Vec (SG)} & \textbf{1.00} & \textbf{0.97} & \textbf{0.94} & \textbf{0.91} & &  \textbf{1.00} & \textbf{0.90} & \textbf{0.92} & \underline{0.86} \\
            \textbf{Word2Vec (CB)} & 0.70 & 0.83 & 0.86 & 0.84 & &  \textbf{1.00} & {0.83} & 0.82 & 0.73 \\
            \textbf{CantReader~\cite{cantreader}} & 0.80 & 0.60 & 0.40 & 0.30 & & 0.80 & 0.67 & 0.56 & 0.42 \\
            \textbf{Zhu et al.~\cite{zhu2021self}} & \underline{0.90} & 0.77 & 0.68 & 0.54 & & 0.90 & 0.73 & 0.70 & 0.56 \\
            \midrule
            \textbf{\model{}} & \underline{0.90} & \underline{0.93} & \underline{0.92} & \underline{0.88} & & 0.80 & \textbf{0.90} & \underline{0.90} & \textbf{0.89} \\
            \bottomrule
        \end{tabular}%
    % }
    \label{tab:evaluation2}
\end{table*}


==> Tables/extended_seed_terms.tex <==
\begin{table*}[t]
    \centering
    \caption{Additional drug seed terms taken from jargon extraction.}
    \small
    % \tiny
    % \resizebox{0.9\linewidth}{!}{%
        \begin{tabular} {c c c c c c c}
            \toprule
            \multicolumn{7}{c}{\textbf{Added Drug Seed Terms}} \\
            \midrule
            ambien & amphetamines & ativan & benadryl & codeine & diazepam & dph \\
            dxm & etizolam & gabapentin & ket & kratom & lsa & md \\
            melatonin & methylone & modafinil & mxe & phenibut & shroom & tramadol \\
            valium & vyvanse & xtc \\
            \bottomrule   
        \end{tabular}
    % }
    \label{tab:added_drug_seed_terms}
\end{table*}

==> Tables/extracted_word_top100.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Top 100 extracted illicit drug jargons from each approaches.}
%     % \footnotesize
%     \scriptsize
%     % \resizebox{\linewidth}{!}{%
%         \begin{tabular} {l c c c c c c c c c c c c c c c c}
%             \toprule
%             \textbf{Apporach} & \multicolumn{16}{c}{\textbf{Top 100 extracted illicit drug jargons}} \\
%             \midrule
%             \textbf{Ours} & acid & weed & dxm & shrooms & coke & kratom & dmt & alcohol & meth & mxe & psychedelics & vyvanse & cannabis & phenibut & dph & etizolam \\ 
% & mushrooms & benzos & caffeine & tramadol & opiates & codeine & valium & speed & salvia & amphetamines & pot & modafinil & ket & ambien & shroom & benadryl \\ 
% & thc & mda & h & md & k & lsa & gabapentin & bud & melatonin & benzo & stimulants & diazepam & pills & ativan & methylone & xtc \\ 
% & oxy & tobacco & mephedrone & zoloft & focalin & wellbutrin & diphenhydramine & prozac & dope & methadone & dexedrine & stims & mushroom & ayahuasca & seroquel & clonazolam \\ 
% & edibles & lucy & xans & spice & stuff & lorazepam & opioids & lexapro & fent & hydro & ibuprofen & lyrica & ecstacy & addy & theanine & psilocybin \\ 
% & powder & etiz & product & nicotine & opiate & cigarettes & shatter & crack & dom & pill & psychs & alp & booze & tylenol & tabs & mdpv \\ 
% & amt & dpt & magnesium & ssris\\
%             % \textbf{Word2Vec (SG)} & \\
%             % \textbf{CantReader} & \\
%             % \textbf{S&P} & \\
%             \bottomrule   
%         \end{tabular}%
%     % }
%     \label{tab:top100_word_list}
% \end{table*}

% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table*}[t]
    \centering
    \caption{Top 100 extracted drug jargon from each approach. Correctly extracted drug jargon terms are colored \textcolor{Brown}{brown}. We excluded `drug' and `drugs' for clarity and redundancy reasons.}
    % \footnotesize
    \scriptsize
    % \resizebox{\linewidth}{!}{%
    % {\normalsize
        \begin{tabular} {l p{0.8\linewidth}}
            \toprule
            {\small \textbf{}} &  \multicolumn{1}{c}{\small \textbf{Top 100 extracted drug jargon}}\\
            \midrule
            {\small \textbf{\model{}}} &  
            {\small \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{dxm}}, \textcolor{Brown}{\textbf{weed}}, \textcolor{Brown}{\textbf{shrooms}}, \textcolor{Brown}{\textbf{coke}}, \textcolor{Brown}{\textbf{kratom}}, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{dmt}}, alcohol, \textcolor{Brown}{\textbf{mxe}}, \textcolor{Brown}{\textbf{psychedelics}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{dph}}, \textcolor{Brown}{\textbf{phenibut}}, caffeine, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{benzos}}, \textcolor{Brown}{\textbf{opiates}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{salvia}}, \textcolor{Brown}{\textbf{speed}}, \textcolor{Brown}{\textbf{amphetamines}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{modafinil}}, \textcolor{Brown}{\textbf{shroom}}, \textcolor{Brown}{\textbf{benadryl}}, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{ket}}, \textcolor{Brown}{\textbf{mda}}, \textcolor{Brown}{\textbf{thc}}, \textcolor{Brown}{\textbf{h}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{gabapentin}}, \textcolor{Brown}{\textbf{k}}, \textcolor{Brown}{\textbf{md}}, melatonin, \textcolor{Brown}{\textbf{stimulants}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{mephedrone}}, \textcolor{Brown}{\textbf{zoloft}}, \textcolor{Brown}{\textbf{methylone}}, \textcolor{Brown}{\textbf{diphenhydramine}}, \textcolor{Brown}{\textbf{xtc}}, \textcolor{Brown}{\textbf{methadone}}, \textcolor{Brown}{\textbf{prozac}}, \textcolor{Brown}{\textbf{pills}}, \textcolor{Brown}{\textbf{wellbutrin}}, tobacco, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{benzo}}, \textcolor{Brown}{\textbf{mushroom}}, \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{ayahuasca}}, \textcolor{Brown}{\textbf{stims}}, \textcolor{Brown}{\textbf{clonazolam}}, \textcolor{Brown}{\textbf{seroquel}}, \textcolor{Brown}{\textbf{dope}}, \textcolor{Brown}{\textbf{lexapro}}, \textcolor{Brown}{\textbf{lucy}}, \textcolor{Brown}{\textbf{bud}}, \textcolor{Brown}{\textbf{xans}}, \textcolor{Brown}{\textbf{spice}}, \textcolor{Brown}{\textbf{psilocybin}}, \textcolor{Brown}{\textbf{opioids}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{lyrica}}, \textcolor{Brown}{\textbf{crack}}, \textcolor{Brown}{\textbf{edibles}}, \textcolor{Brown}{\textbf{bath}}, \textcolor{Brown}{\textbf{magnesium}}, \textcolor{Brown}{\textbf{hydro}}, \textcolor{Brown}{\textbf{ssris}}, \textcolor{Brown}{\textbf{etiz}}, \textcolor{Brown}{\textbf{addy}}, \textcolor{Brown}{\textbf{mdpv}}, ibuprofen, \textcolor{Brown}{\textbf{dom}}, nicotine, \textcolor{Brown}{\textbf{effexor}}, \textcolor{Brown}{\textbf{ecstacy}}, acetaminophen, \textcolor{Brown}{\textbf{psychs}}, cigarettes, \textcolor{Brown}{\textbf{amt}}, viagra, \textcolor{Brown}{\textbf{opiate}}, \textcolor{Brown}{\textbf{pregabalin}}, booze, paracetamol, \textcolor{Brown}{\textbf{dpt}}, \textcolor{Brown}{\textbf{alp}}, \textcolor{Brown}{\textbf{datura}}, \textcolor{Brown}{\textbf{benzodiazepines}}}\\
            % {\small acid, weed, dxm, shrooms, coke, kratom, dmt, alcohol, meth, mxe, \textbf{psychedelics}, vyvanse, cannabis, phenibut, dph, etizolam, mushrooms, benzos, caffeine, tramadol, opiates, codeine, valium, speed, salvia, amphetamines, pot, modafinil, ket, ambien, shroom, benadryl, thc, mda, h, md, k, lsa, gabapentin, bud, melatonin, benzo, stimulants, diazepam, pills, ativan, methylone, xtc, oxy, tobacco, mephedrone, zoloft, focalin, wellbutrin, diphenhydramine, prozac, dope, methadone, dexedrine, stims, mushroom, ayahuasca, seroquel, clonazolam, edibles, lucy, xans, spice, stuff, lorazepam, opioids, lexapro, fent, hydro, ibuprofen, lyrica, ecstacy, addy, theanine, psilocybin, powder, etiz, product, nicotine, opiate, cigarettes, shatter, crack, dom, pill, psychs, alp, booze, tylenol, tabs, mdpv, amt, dpt, magnesium, ssris}\\
            % \midrule
            % {\small \textbf{Word2Vec (SG)}} & {\small \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{heroine}}, \textcolor{Brown}{\textbf{adderal}}, \textcolor{Brown}{\textbf{hydros}}, \textcolor{Brown}{\textbf{amph}}, \textcolor{Brown}{\textbf{prometh}}, \textcolor{Brown}{\textbf{aderall}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{vicoden}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{seroquel}}, \textcolor{Brown}{\textbf{percs}}, \textcolor{Brown}{\textbf{zopiclone}}, \textcolor{Brown}{\textbf{oxazepam}}, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{kpin}}, \textcolor{Brown}{\textbf{xan}}, \textcolor{Brown}{\textbf{gabapentin}}, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{meo}}, \textcolor{Brown}{\textbf{gbl}}, \textcolor{Brown}{\textbf{percocets}}, syrup, \textcolor{Brown}{\textbf{shrooms}}, \textcolor{Brown}{\textbf{kpins}}, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{clonazolam}}, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{norcos}}, ir, \textcolor{Brown}{\textbf{oxymorphone}}, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{xans}}, \textcolor{Brown}{\textbf{etiz}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{carfentanil}}, \textcolor{Brown}{\textbf{vyvance}}, xr, \textcolor{Brown}{\textbf{nbome}}, \textcolor{Brown}{\textbf{codiene}}, \textcolor{Brown}{\textbf{lortab}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{mescalin}}, \textcolor{Brown}{\textbf{ecstacy}}, \textcolor{Brown}{\textbf{opana}}, \textcolor{Brown}{\textbf{alp}}, \textcolor{Brown}{\textbf{ketaset}}, sulfate, \textcolor{Brown}{\textbf{mesc}}, \textcolor{Brown}{\textbf{subutex}}, phenergan, \textcolor{Brown}{\textbf{ephedrine}}, \textcolor{Brown}{\textbf{dexamphetamine}}, \textcolor{Brown}{\textbf{etaqualone}}, dextrose, \textcolor{Brown}{\textbf{mj}}, sulphate, \textcolor{Brown}{\textbf{methadone}}, \textcolor{Brown}{\textbf{lad}}, \textcolor{Brown}{\textbf{aco}}, \textcolor{Brown}{\textbf{coke}}, \textcolor{Brown}{\textbf{dmt}}, \textcolor{Brown}{\textbf{nbomes}}, \textcolor{Brown}{\textbf{alpraz}}, \textcolor{Brown}{\textbf{bupe}}, \textcolor{Brown}{\textbf{alprozolam}}, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{poppy}}, \textcolor{Brown}{\textbf{stimulant}}, \textcolor{Brown}{\textbf{triprolidine}}, \textcolor{Brown}{\textbf{sass}}, \textcolor{Brown}{\textbf{cheratussin}}, \textcolor{Brown}{\textbf{temazepam}}, \textcolor{Brown}{\textbf{herion}}, \textcolor{Brown}{\textbf{butyr}}, linctus, \textcolor{Brown}{\textbf{psychedelics}}, \textcolor{Brown}{\textbf{tussionex}}, \textcolor{Brown}{\textbf{cb}}, milliliters, \textcolor{Brown}{\textbf{mxe}}, \textcolor{Brown}{\textbf{nyquil}}, \textcolor{Brown}{\textbf{ayahuasca}}, \textcolor{Brown}{\textbf{lsz}}, \textcolor{Brown}{\textbf{fetanyl}}, \textcolor{Brown}{\textbf{roxy}}, \textcolor{Brown}{\textbf{mda}}, \textcolor{Brown}{\textbf{amphet}}, \textcolor{Brown}{\textbf{amanita}}, \textcolor{Brown}{\textbf{cactus}}, \textcolor{Brown}{\textbf{naphyrone}}, \textcolor{Brown}{\textbf{xtc}}}\\
            % {\small \textbf{Word2Vec (SG)}} & {\small dexedrine, vyvanse, fent, ativan, lorazepam, heroine, adderal, hydros, amph, prometh, aderall, diazepam, vicoden, focalin, seroquel, percs, zopiclone, oxazepam, tramadol, kpin, xan, gabapentin, etizolam, codeine, acid, valium, meo, gbl, percocets, syrup, shrooms, kpins, oxy, clonazolam, ambien, norcos, ir, oxymorphone, meth, lsa, xans, etiz, pot, carfentanil, vyvance, xr, nbome, codiene, lortab, cannabis, mescalin, ecstacy, opana, alp, ketaset, sulfate, mesc, subutex, phenergan, ephedrine, dexamphetamine, etaqualone, dextrose, mj, sulphate, methadone, lad, aco, coke, dmt, nbomes, alpraz, bupe, alprozolam, mushrooms, poppy, stimulant, triprolidine, sass, cheratussin, temazepam, herion, butyr, linctus, psychedelics, tussionex, cb, milliliters, mxe, nyquil, ayahuasca, lsz, fetanyl, roxy, mda, amphet, amanita, cactus, naphyrone, xtc}\\
            \midrule
            {\small \textbf{Word2Vec~\cite{mikolov2013efficient}}} & {\small actavis, \textcolor{Brown}{\textbf{roxycodone}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{roxy}}, mundipharma, \textcolor{Brown}{\textbf{ksalol}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{methadone}}, roche, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{roxies}}, \textcolor{Brown}{\textbf{cenforce}}, \textcolor{Brown}{\textbf{nitrazepam}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{dihydrocodeine}}, transdermal, xr, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{diluadid}}, \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{cacti}}, \textcolor{Brown}{\textbf{ultram}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{seconal}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{oxymorphone}}, \textcolor{Brown}{\textbf{opana}}, \textcolor{Brown}{\textbf{zolpidem}}, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{percs}}, \textcolor{Brown}{\textbf{coke}}, \textcolor{Brown}{\textbf{lunesta}}, \textcolor{Brown}{\textbf{amanita}}, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{muscaria}}, \textcolor{Brown}{\textbf{norcos}}, \textcolor{Brown}{\textbf{modafinil}}, psychotria, syrup, \textcolor{Brown}{\textbf{spores}}, \textcolor{Brown}{\textbf{endone}}, \textcolor{Brown}{\textbf{carisoprodol}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{methoxetamine}}, \textcolor{Brown}{\textbf{subutex}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{methedrone}}, \textcolor{Brown}{\textbf{triazolam}}, \textcolor{Brown}{\textbf{methyphenidate}}, \textcolor{Brown}{\textbf{adderal}}, \textcolor{Brown}{\textbf{ayahuasca}}, lophophora, \textcolor{Brown}{\textbf{cyclobenzaprine}}, \textcolor{Brown}{\textbf{gbl}}, \textcolor{Brown}{\textbf{zopiclone}}, \textcolor{Brown}{\textbf{mipt}}, \textcolor{Brown}{\textbf{prometh}}, \textcolor{Brown}{\textbf{modvigil}}, \textcolor{Brown}{\textbf{cheratussin}}, \textcolor{Brown}{\textbf{duragesic}}, \textcolor{Brown}{\textbf{cactus}}, \textcolor{Brown}{\textbf{desoxyn}}, \textcolor{Brown}{\textbf{cannavis}}, \textcolor{Brown}{\textbf{mitragyna}}, acacia, \textcolor{Brown}{\textbf{naphyrone}}, indigenous, \textcolor{Brown}{\textbf{apvp}}, \textcolor{Brown}{\textbf{marajuana}}, \textcolor{Brown}{\textbf{diacetylmorphine}}, \textcolor{Brown}{\textbf{harmine}}, endogenous, phenergan, \textcolor{Brown}{\textbf{dex}}, \textcolor{Brown}{\textbf{buprenorphine}}, barbital, \textcolor{Brown}{\textbf{lsh}}, \textcolor{Brown}{\textbf{ctmp}}, teva, potentates, \textcolor{Brown}{\textbf{mj}}, \textcolor{Brown}{\textbf{tramadols}}, \textcolor{Brown}{\textbf{carfentanil}}, \textcolor{Brown}{\textbf{cannibas}}, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{heroine}}, \textcolor{Brown}{\textbf{hemp}}, \textcolor{Brown}{\textbf{dmt}}, \textcolor{Brown}{\textbf{speciosa}}, \textcolor{Brown}{\textbf{poppy}}, bolivia, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{cbds}}, \textcolor{Brown}{\textbf{adderalls}}, \textcolor{Brown}{\textbf{marihuana}}, \textcolor{Brown}{\textbf{alp}}, \textcolor{Brown}{\textbf{ephedra}}, \textcolor{Brown}{\textbf{leaf}}}\\
            \midrule
            % {\small \textbf{CantReader~\cite{cantreader}}} & {\small tramadol, lyrica, codeine, oxy, diazepam, valium, viagra, ambien, bud, ibuprofen, modafinil, dos, meth, instagram, facebook, nugs, zoloft, soma, nug, synthetic, dxm, unpause, wantz, cannabinoids, kush, superawesome, opiate, asterix, promess, snapchat, hashish, rat, nika, getit, comfused, fanx, citalopram, whacha, medication, laughted, fraid, nappa, janel, chrome, pica, spotify, years, fluked, dartboard, theys, niceeeeeee, unfriend, pregnent, waterblocks, bahahahahah, norcos, pharmaceutical, rakesh, painkiller, ayyye, rupaul, safezone, enver, percs, cooool, luffy, particpate, apprieciate, othere, whatttttt, tamara, brogue, mendel, blist, vanned, worrying, skype, cannabis, focalin, iv, opioid, waaaayy, squealer, skan, uhhhm, dex, kneegrow, plagiarist, benzo, alembic, prescribed, minecraft, lisbeth, weed, anticheat, jesuschrist, stimulant, whoooole, suuuuuure, johor}\\
            {\small \textbf{CantReader~\cite{cantreader}}} & {\small \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{lyrica}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{valium}}, viagra, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{bud}}, ibuprofen, \textcolor{Brown}{\textbf{modafinil}}, dos, \textcolor{Brown}{\textbf{meth}}, instagram, facebook, \textcolor{Brown}{\textbf{nugs}}, \textcolor{Brown}{\textbf{zoloft}}, \textcolor{Brown}{\textbf{soma}}, \textcolor{Brown}{\textbf{nug}}, synthetic, \textcolor{Brown}{\textbf{dxm}}, unpause, wantz, \textcolor{Brown}{\textbf{cannabinoids}}, \textcolor{Brown}{\textbf{kush}}, superawesome, \textcolor{Brown}{\textbf{opiate}}, asterix, promess, snapchat, \textcolor{Brown}{\textbf{hashish}}, rat, nika, getit, comfused, fanx, \textcolor{Brown}{\textbf{citalopram}}, whacha, medication, laughted, fraid, nappa, janel, chrome, pica, spotify, years, fluked, dartboard, theys, niceeeeeee, unfriend, pregnent, waterblocks, bahahahahah, \textcolor{Brown}{\textbf{norcos}}, pharmaceutical, rakesh, \textcolor{Brown}{\textbf{painkiller}}, ayyye, rupaul, safezone, enver, \textcolor{Brown}{\textbf{percs}}, cooool, luffy, particpate, apprieciate, othere, whatttttt, tamara, brogue, mendel, blist, vanned, worrying, skype, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{focalin}}, iv, \textcolor{Brown}{\textbf{opioid}}, waaaayy, squealer, skan, uhhhm, \textcolor{Brown}{\textbf{dex}}, kneegrow, plagiarist, \textcolor{Brown}{\textbf{benzo}}, alembic, prescribed, minecraft, lisbeth, \textcolor{Brown}{\textbf{weed}}, anticheat, jesuschrist, \textcolor{Brown}{\textbf{stimulant}}, whoooole, suuuuuure, johor}\\
            \midrule
            % {\small \textbf{Zhu et al.~\cite{zhu2021self}}} & {\small weed, coke, alcohol, acid, cannabis, speed, mushrooms, md, crack, pot, pills, something, k, hydro, h, l, lean, powder, tobacco, e, benz, hash, blow, met, crystal, cigarettes, lithium, others, lucy, amp, sh, narcotics, spice, ir, anything, heroine, magnesium, x, rita, bud, psychedelic, shit, substance, water, add, coffee, stuff, bars, sex, pill, vodka, mx, medication, ox, rc, daily, oil, smoking, one, beer, gold, dom, product, dex, antibiotics, substances, op, coca, recreational, doc, cid, money, ether, roxy, 2, anxiety, tar, testosterone, ice, wax, white, ethanol, addiction, oral, drinking, music, mandy, sugar, syrup, m1, shatter, pharmaceuticals, depression, code, prescription, pure, bk, rolling, tea, synthetic}\\
            {\small \textbf{Zhu et al.~\cite{zhu2021self}}} & {\small \textcolor{Brown}{\textbf{weed}}, \textcolor{Brown}{\textbf{coke}}, alcohol, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{speed}}, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{md}}, \textcolor{Brown}{\textbf{crack}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{pills}}, something, \textcolor{Brown}{\textbf{k}}, \textcolor{Brown}{\textbf{hydro}}, \textcolor{Brown}{\textbf{h}}, \textcolor{Brown}{\textbf{l}}, \textcolor{Brown}{\textbf{lean}}, \textcolor{Brown}{\textbf{powder}}, tobacco, \textcolor{Brown}{\textbf{e}}, \textcolor{Brown}{\textbf{benz}}, \textcolor{Brown}{\textbf{hash}}, \textcolor{Brown}{\textbf{blow}}, met, \textcolor{Brown}{\textbf{crystal}}, cigarettes, lithium, others, \textcolor{Brown}{\textbf{lucy}}, \textcolor{Brown}{\textbf{amp}}, sh, \textcolor{Brown}{\textbf{narcotics}}, \textcolor{Brown}{\textbf{spice}}, ir, anything, \textcolor{Brown}{\textbf{heroine}}, \textcolor{Brown}{\textbf{magnesium}}, \textcolor{Brown}{\textbf{x}}, \textcolor{Brown}{\textbf{rita}}, \textcolor{Brown}{\textbf{bud}}, \textcolor{Brown}{\textbf{psychedelic}}, shit, substance, \textcolor{Brown}{\textbf{water}}, add, coffee, stuff, \textcolor{Brown}{\textbf{bars}}, sex, \textcolor{Brown}{\textbf{pill}}, vodka, mx, medication, \textcolor{Brown}{\textbf{ox}}, \textcolor{Brown}{\textbf{rc}}, daily, \textcolor{Brown}{\textbf{oil}}, smoking, one, beer, \textcolor{Brown}{\textbf{gold}}, \textcolor{Brown}{\textbf{dom}}, product, \textcolor{Brown}{\textbf{dex}}, antibiotics, substances, \textcolor{Brown}{\textbf{op}}, \textcolor{Brown}{\textbf{coca}}, recreational, doc, \textcolor{Brown}{\textbf{cid}}, money, ether, \textcolor{Brown}{\textbf{roxy}}, 2, anxiety, \textcolor{Brown}{\textbf{tar}}, testosterone, \textcolor{Brown}{\textbf{ice}}, \textcolor{Brown}{\textbf{wax}}, \textcolor{Brown}{\textbf{white}}, ethanol, addiction, oral, drinking, music, \textcolor{Brown}{\textbf{mandy}}, sugar, syrup, \textcolor{Brown}{\textbf{m1}}, \textcolor{Brown}{\textbf{shatter}}, pharmaceuticals, depression, code, prescription, \textcolor{Brown}{\textbf{pure}}, \textcolor{Brown}{\textbf{bk}}, \textcolor{Brown}{\textbf{rolling}}, tea, synthetic}\\
            \bottomrule   
        \end{tabular}%
        % }
    % }
    \label{tab:top100_word_list}
\end{table*}




==> Tables/extracted_word_top30.tex <==
\begin{table*}[t]
    \centering
    \caption{Top 30 extracted drug jargon from each approach. Correctly extracted jargon terms are colored \textcolor{Brown}{brown}.}
    % \footnotesize
    \scriptsize
    % \resizebox{\linewidth}{!}{%
    % {\normalsize
        \begin{tabular} {l p{0.8\linewidth}}
            \toprule
            {\small \textbf{}} &  \multicolumn{1}{c}{\small \textbf{Top 30 extracted drug jargon}}\\
            \midrule
            {\small \textbf{\model{}}} &  
            {\footnotesize \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{weed}}, \textcolor{Brown}{\textbf{dxm}}, \textcolor{Brown}{\textbf{shrooms}}, \textcolor{Brown}{\textbf{coke}}, \textcolor{Brown}{\textbf{kratom}}, \textcolor{Brown}{\textbf{dmt}}, alcohol, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{mxe}}, \textcolor{Brown}{\textbf{psychedelics}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{phenibut}}, \textcolor{Brown}{\textbf{dph}}, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{benzos}}, caffeine, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{opiates}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{speed}}, \textcolor{Brown}{\textbf{salvia}}, \textcolor{Brown}{\textbf{amphetamines}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{modafinil}}, \textcolor{Brown}{\textbf{ket}}, \textcolor{Brown}{\textbf{ambien}}}\\
            \midrule
            {\small \textbf{Word2Vec (SG)}} & {\footnotesize \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{heroine}}, \textcolor{Brown}{\textbf{adderal}}, \textcolor{Brown}{\textbf{hydros}}, \textcolor{Brown}{\textbf{amph}}, \textcolor{Brown}{\textbf{prometh}}, \textcolor{Brown}{\textbf{aderall}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{vicoden}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{seroquel}}, \textcolor{Brown}{\textbf{percs}}, \textcolor{Brown}{\textbf{zopiclone}}, \textcolor{Brown}{\textbf{oxazepam}}, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{kpin}}, \textcolor{Brown}{\textbf{xan}}, \textcolor{Brown}{\textbf{gabapentin}}, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{meo}}, \textcolor{Brown}{\textbf{gbl}}, \textcolor{Brown}{\textbf{percocets}}, syrup}\\

            \midrule
            {\small \textbf{Word2Vec (CB)}} & {\footnotesize actavis, \textcolor{Brown}{\textbf{roxycodone}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{roxy}}, mundipharma, \textcolor{Brown}{\textbf{ksalol}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{methadone}}, roche, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{roxies}}, \textcolor{Brown}{\textbf{cenforce}}, \textcolor{Brown}{\textbf{nitrazepam}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{dihydrocodeine}}, transdermal, xr, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{diluadid}}, \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{cacti}}, \textcolor{Brown}{\textbf{ultram}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{seconal}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{oxymorphone}}, \textcolor{Brown}{\textbf{opana}}, \textcolor{Brown}{\textbf{zolpidem}}}\\
            \midrule
            {\small \textbf{CantReader~\cite{cantreader}}} & {\footnotesize \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{lyrica}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{valium}}, viagra, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{bud}}, ibuprofen, \textcolor{Brown}{\textbf{modafinil}}, dos, \textcolor{Brown}{\textbf{meth}}, instagram, facebook, \textcolor{Brown}{\textbf{nugs}}, \textcolor{Brown}{\textbf{zoloft}}, \textcolor{Brown}{\textbf{soma}}, \textcolor{Brown}{\textbf{nug}}, synthetic, \textcolor{Brown}{\textbf{dxm}}, unpause, wantz, \textcolor{Brown}{\textbf{cannabinoids}}, \textcolor{Brown}{\textbf{kush}}, superawesome, \textcolor{Brown}{\textbf{opiate}}, asterix, promess, snapchat}\\
            \midrule
            {\small \textbf{Zhu et al.~\cite{zhu2021self}}} & {\footnotesize \textcolor{Brown}{\textbf{weed}}, \textcolor{Brown}{\textbf{coke}}, alcohol, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{speed}}, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{md}}, \textcolor{Brown}{\textbf{crack}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{pills}}, something, \textcolor{Brown}{\textbf{k}}, \textcolor{Brown}{\textbf{hydro}}, \textcolor{Brown}{\textbf{h}}, \textcolor{Brown}{\textbf{l}}, \textcolor{Brown}{\textbf{lean}}, \textcolor{Brown}{\textbf{powder}}, tobacco, \textcolor{Brown}{\textbf{e}}, \textcolor{Brown}{\textbf{benz}}, \textcolor{Brown}{\textbf{hash}}, \textcolor{Brown}{\textbf{blow}}, met, \textcolor{Brown}{\textbf{crystal}}, cigarettes, lithium, others, \textcolor{Brown}{\textbf{lucy}}, \textcolor{Brown}{\textbf{amp}}}\\
            \bottomrule   
        \end{tabular}%
        % }
    % }
    \label{tab:top30_word_list}
\end{table*}




==> Tables/extracted_word_top50.tex <==
\begin{table*}[t]
    \centering
    \caption{Top 50 extracted drug jargon from each system. Correctly extracted drug jargon terms are colored \textcolor{Brown}{brown}.}
    % \footnotesize
    \scriptsize
    % \resizebox{\linewidth}{!}{%
    % {\normalsize
        \begin{tabular} {l p{0.8\linewidth}}
            \toprule
            {\small \textbf{}} &  \multicolumn{1}{c}{\small \textbf{Top 50 extracted drug jargon}}\\
            \midrule
            {\small \textbf{\model{}}} &  
            {\small \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{weed}}, \textcolor{Brown}{\textbf{dxm}}, \textcolor{Brown}{\textbf{shrooms}}, \textcolor{Brown}{\textbf{coke}}, \textcolor{Brown}{\textbf{kratom}}, \textcolor{Brown}{\textbf{dmt}}, alcohol, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{mxe}}, \textcolor{Brown}{\textbf{psychedelics}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{phenibut}}, \textcolor{Brown}{\textbf{dph}}, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{benzos}}, caffeine, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{opiates}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{speed}}, \textcolor{Brown}{\textbf{salvia}}, \textcolor{Brown}{\textbf{amphetamines}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{modafinil}}, \textcolor{Brown}{\textbf{ket}}, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{shroom}}, \textcolor{Brown}{\textbf{benadryl}}, \textcolor{Brown}{\textbf{thc}}, \textcolor{Brown}{\textbf{mda}}, \textcolor{Brown}{\textbf{h}}, \textcolor{Brown}{\textbf{md}}, \textcolor{Brown}{\textbf{k}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{gabapentin}}, \textcolor{Brown}{\textbf{bud}}, melatonin, \textcolor{Brown}{\textbf{benzo}}, \textcolor{Brown}{\textbf{stimulants}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{pills}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{methylone}}, \textcolor{Brown}{\textbf{xtc}}, \textcolor{Brown}{\textbf{oxy}}, tobacco}\\
            \midrule
            {\small \textbf{Word2Vec (SG)}} & {\small \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{heroine}}, \textcolor{Brown}{\textbf{adderal}}, \textcolor{Brown}{\textbf{hydros}}, \textcolor{Brown}{\textbf{amph}}, \textcolor{Brown}{\textbf{prometh}}, \textcolor{Brown}{\textbf{aderall}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{vicoden}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{seroquel}}, \textcolor{Brown}{\textbf{percs}}, \textcolor{Brown}{\textbf{zopiclone}}, \textcolor{Brown}{\textbf{oxazepam}}, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{kpin}}, \textcolor{Brown}{\textbf{xan}}, \textcolor{Brown}{\textbf{gabapentin}}, \textcolor{Brown}{\textbf{etizolam}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{meo}}, \textcolor{Brown}{\textbf{gbl}}, \textcolor{Brown}{\textbf{percocets}}, syrup, \textcolor{Brown}{\textbf{shrooms}}, \textcolor{Brown}{\textbf{kpins}}, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{clonazolam}}, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{norcos}}, ir, \textcolor{Brown}{\textbf{oxymorphone}}, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{xans}}, \textcolor{Brown}{\textbf{etiz}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{carfentanil}}, \textcolor{Brown}{\textbf{vyvance}}, xr, \textcolor{Brown}{\textbf{nbome}}, \textcolor{Brown}{\textbf{codiene}}, \textcolor{Brown}{\textbf{lortab}}, \textcolor{Brown}{\textbf{cannabis}}}\\

            \midrule
            {\small \textbf{Word2Vec (CB)}} & {\small actavis, \textcolor{Brown}{\textbf{roxycodone}}, \textcolor{Brown}{\textbf{fent}}, \textcolor{Brown}{\textbf{roxy}}, mundipharma, \textcolor{Brown}{\textbf{ksalol}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{ativan}}, \textcolor{Brown}{\textbf{methadone}}, roche, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{roxies}}, \textcolor{Brown}{\textbf{cenforce}}, \textcolor{Brown}{\textbf{nitrazepam}}, \textcolor{Brown}{\textbf{lorazepam}}, \textcolor{Brown}{\textbf{dihydrocodeine}}, transdermal, xr, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{diluadid}}, \textcolor{Brown}{\textbf{dexedrine}}, \textcolor{Brown}{\textbf{cacti}}, \textcolor{Brown}{\textbf{ultram}}, \textcolor{Brown}{\textbf{focalin}}, \textcolor{Brown}{\textbf{vyvanse}}, \textcolor{Brown}{\textbf{seconal}}, \textcolor{Brown}{\textbf{lsa}}, \textcolor{Brown}{\textbf{oxymorphone}}, \textcolor{Brown}{\textbf{opana}}, \textcolor{Brown}{\textbf{zolpidem}}, \textcolor{Brown}{\textbf{meth}}, \textcolor{Brown}{\textbf{percs}}, \textcolor{Brown}{\textbf{coke}}, \textcolor{Brown}{\textbf{lunesta}}, \textcolor{Brown}{\textbf{amanita}}, \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{muscaria}}, \textcolor{Brown}{\textbf{norcos}}, \textcolor{Brown}{\textbf{modafinil}}, psychotria, syrup, \textcolor{Brown}{\textbf{spores}}, \textcolor{Brown}{\textbf{endone}}, \textcolor{Brown}{\textbf{carisoprodol}}, \textcolor{Brown}{\textbf{valium}}, \textcolor{Brown}{\textbf{methoxetamine}}, \textcolor{Brown}{\textbf{subutex}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{methedrone}}, \textcolor{Brown}{\textbf{triazolam}}}\\
            \midrule
            {\small \textbf{CantReader~\cite{cantreader}}} & {\small \textcolor{Brown}{\textbf{tramadol}}, \textcolor{Brown}{\textbf{lyrica}}, \textcolor{Brown}{\textbf{codeine}}, \textcolor{Brown}{\textbf{oxy}}, \textcolor{Brown}{\textbf{diazepam}}, \textcolor{Brown}{\textbf{valium}}, viagra, \textcolor{Brown}{\textbf{ambien}}, \textcolor{Brown}{\textbf{bud}}, ibuprofen, \textcolor{Brown}{\textbf{modafinil}}, dos, \textcolor{Brown}{\textbf{meth}}, instagram, facebook, \textcolor{Brown}{\textbf{nugs}}, \textcolor{Brown}{\textbf{zoloft}}, \textcolor{Brown}{\textbf{soma}}, \textcolor{Brown}{\textbf{nug}}, synthetic, \textcolor{Brown}{\textbf{dxm}}, unpause, wantz, \textcolor{Brown}{\textbf{cannabinoids}}, \textcolor{Brown}{\textbf{kush}}, superawesome, \textcolor{Brown}{\textbf{opiate}}, asterix, promess, snapchat, \textcolor{Brown}{\textbf{hashish}}, rat, nika, getit, comfused, fanx, \textcolor{Brown}{\textbf{citalopram}}, whacha, medication, laughted, fraid, nappa, janel, chrome, pica, spotify, years, fluked, dartboard, theys}\\
            \midrule
            {\small \textbf{Zhu et al.~\cite{zhu2021self}}} & {\small \textcolor{Brown}{\textbf{weed}}, \textcolor{Brown}{\textbf{coke}}, alcohol, \textcolor{Brown}{\textbf{acid}}, \textcolor{Brown}{\textbf{cannabis}}, \textcolor{Brown}{\textbf{speed}}, \textcolor{Brown}{\textbf{mushrooms}}, \textcolor{Brown}{\textbf{md}}, \textcolor{Brown}{\textbf{crack}}, \textcolor{Brown}{\textbf{pot}}, \textcolor{Brown}{\textbf{pills}}, something, \textcolor{Brown}{\textbf{k}}, \textcolor{Brown}{\textbf{hydro}}, \textcolor{Brown}{\textbf{h}}, \textcolor{Brown}{\textbf{l}}, \textcolor{Brown}{\textbf{lean}}, \textcolor{Brown}{\textbf{powder}}, tobacco, \textcolor{Brown}{\textbf{e}}, \textcolor{Brown}{\textbf{benz}}, \textcolor{Brown}{\textbf{hash}}, \textcolor{Brown}{\textbf{blow}}, met, \textcolor{Brown}{\textbf{crystal}}, cigarettes, lithium, others, \textcolor{Brown}{\textbf{lucy}}, \textcolor{Brown}{\textbf{amp}}, sh, \textcolor{Brown}{\textbf{narcotics}}, \textcolor{Brown}{\textbf{spice}}, ir, anything, \textcolor{Brown}{\textbf{heroine}}, \textcolor{Brown}{\textbf{magnesium}}, \textcolor{Brown}{\textbf{x}}, \textcolor{Brown}{\textbf{rita}}, \textcolor{Brown}{\textbf{bud}}, \textcolor{Brown}{\textbf{psychedelic}}, shit, substance, \textcolor{Brown}{\textbf{water}}, add, coffee, stuff, \textcolor{Brown}{\textbf{bars}}, sex, \textcolor{Brown}{\textbf{pill}}}\\
            \bottomrule   
        \end{tabular}%
        % }
    % }
    \label{tab:top50_word_list}
\end{table*}




==> Tables/sexual_terms.tex <==
\begin{table*}[t]
    \centering
    \caption{Sexual terms used for the pilot experiment. Randomly sampled 10 terms are used as test terms.}
    \scriptsize
    \resizebox{0.9\linewidth}{!}{%
        \begin{tabular} {c c c c c c c c c c}
            \toprule
            \multicolumn{10}{c}{\textbf{Sexual Terms}} \\
            \midrule
            fuck & sex & head & ass & gay & porn & bush & hole & dick & pussy \\
            suck & balls & asshole & faggot & cunt & whore & nuts & bust & johnson & bob\\
            screwed & fag & cock & scumbag & bust & homo & ho & queer & anal & slut \\
            69 & dyke & cum & oral & skank & hooker & poof & slit & willy & wiener\\
            weiner & rapey & boob & wanker & booty & wuss & porno & titty & weenie & threesome\\
            cowgirl & breast & genitals \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:sexual_terms}
\end{table*}


==> Tables/target_word_example.tex <==
\begin{table}[t]
    \centering
    \caption{Examples of sentences from the training data with target words in \textbf{bold}.}
    \footnotesize
    % \resizebox{\linewidth}{!}{%
        \begin{tabular} {l c}
            \toprule
            \textbf{Sentence pool} & \textbf{Example} \\
            \midrule
            \multirow{2}{*}{\textbf{\textit{STMS}}} & \textbf{Cocaine} was super clean on the nose and gave a great feeling. \\
                                                     & Cocaine was super clean on the \textbf{nose} and gave a great feeling. \\
            \midrule
            \textbf{\textit{non-STMS}}               & I've searched the \textbf{internet} and can't find anything too helpful. \\
            \bottomrule            
        \end{tabular}%
    % }
    \label{tab:target_word_example}
\end{table}


==> Tables/word_based_comparison.tex <==
\begin{table}[t]
    \centering
    \caption{Comparison of \model{} with baseline jargon extraction systems.}
    % \scriptsize
    \resizebox{0.85\linewidth}{!}{%
    {\normalsize
        \begin{tabular} {p{0.25\linewidth} P{0.25\linewidth} P{0.25\linewidth} P{0.25\linewidth}}
            \toprule
            {\textbf{}} &  { \textbf{Find euphemism}} & { \textbf{Robust to noise}} & { \textbf{Independent to vocabulary}}\\ 
            \midrule
            \textbf{Word2Vec} &  &\checkmark & \checkmark\\
            \midrule
            \textbf{CantReader~\cite{cantreader}} & \checkmark &  & \checkmark\\
            \midrule
            \textbf{Zhu et al.~\cite{zhu2021self}}  & \checkmark & \checkmark &  \\
            \midrule
            \textbf{\model{}}  & \checkmark & \checkmark & \checkmark  \\
            \bottomrule
        \end{tabular}%
    }
    }
    \label{tab:word_based_comparision}
\end{table}


% \begin{table}[t]
%     \centering
%     \caption{Comparison of \model{} with existing word-based content moderation systems.}
%     % \scriptsize
%     \resizebox{\linewidth}{!}{%
%     {\footnotesize
%         \begin{tabular} {p{0.2\linewidth} P{0.2\linewidth} P{0.2\linewidth} P{0.2\linewidth} P{0.2\linewidth}}
%             \toprule
%             {\textbf{}} &  { \textbf{Find euphemism}} & { \textbf{Robust to noise}} & { \textbf{Independent to vocabulary}} & { \textbf{Apply to unseen words}}\\ 
%             \midrule
%             \textbf{Word2Vec} &  &\checkmark & \checkmark &\\
%             \midrule
%             \textbf{CantReader~\cite{cantreader}} & \checkmark &  & \checkmark &\\
%             \midrule
%             \textbf{Zhu et al.~\cite{zhu2021self}}  & \checkmark & \checkmark &  &\checkmark\\
%             \midrule
%             \textbf{\model{}}  & \checkmark & \checkmark & \checkmark & \checkmark \\
%             \bottomrule
%         \end{tabular}%
%     }
%     }

%     \label{tab:word_based_comparision}
% \end{table}
